Benchmarking, Analysis, and Optimization of Serverless Function Snapshots

Serverless computing has seen rapid adoption due to its high scalability and flexible, pay-as-you-go billing model. In serverless, developers structure their services as a collection of functions, sporadically invoked by various events like clicks. High inter-arrival time variability of function invocations motivates the providers to start new function instances upon each invocation, leading to significant cold-start delays that degrade user experience. To reduce cold-start latency, the industry has turned to snapshotting, whereby an image of a fully-booted function is stored on disk, enabling a faster invocation compared to booting a function from scratch. This work introduces vHive, an open-source framework for serverless experimentation with the goal of enabling researchers to study and innovate across the entire serverless stack. Using vHive, we characterize a state-of-the-art snapshot-based serverless infrastructure, based on industry-leading Containerd orchestration framework and Firecracker hypervisor technologies. We find that the execution time of a function started from a snapshot is 95% higher, on average, than when the same function is memory-resident. We show that the high latency is attributable to frequent page faults as the function's state is brought from disk into guest memory one page at a time. Our analysis further reveals that functions access the same stable working set of pages across different invocations of the same function. By leveraging this insight, we build REAP, a light-weight software mechanism for serverless hosts that records functions' stable working set of guest memory pages and proactively prefetches it from disk into memory. Compared to baseline snapshotting, REAP slashes the cold-start delays by 3.7x, on average.

==> 3-infra.tex <==
\section{End-to-End Serverless Infrastructure}
\label{sec:characterization}

\boris{Add a lead-in: we overview general serverless architecture, and describe our open-source infrastructure for at-scale serverless experimentation.}

\subsection{Serverless Architecture Overview}
\label{sec:containerd101}


Serverless systems have a datacenter-scale distributed architecture that comprises an extensive number of components and services (Fig.~\ref{fig:serverless_overview}). The software components are connected with a flexible REST API \boris{define REST} fabric that enables flexible management and resources usage monitoring while delivering high performance.


%\input{floats/fl_serverless_overview}

\boris{Need to make it clear that you're describing a typical industry deployment, not something you cooked up. If you could say that the following is representative of AWS Lambda or Azure Functions, with a citation, that would be perfect.}
A serverless system comprises of the scale-out shared-nothing front-end fleet of servers facing the serverless function invocations, the worker fleet that executes the function code, and the worker manager that connects the two together~\cite{agache:firecracker,shahrad:serverless,krook:openwhisk}.
A function invocation, in a form of a REST API request, first arrives at one of the front-end servers for request authentication and mapping of the request to its corresponding function. 
%Then, the request may follow the slow \emph{control path}, e.g., when no instances of the function are running, or fast \emph{data path}. 

The \emph{worker manager} is a scale-up highly available service that maintains the mapping of the functions to their available instances and manages the fleet of worker servers that run the instances of the function. If no instances of the function are running, the worker manager selects a worker that can start a new instance of the function, based on the current load and available resources of the worker. To facilitate recurring events processing, the worker manager enables sticky routing connecting front-end servers to a minimal number of workers that allows reuse of the already running function instances.

Worker servers feature a highly modular architecture that aims to deliver high performance and security while running thousands of function instances, where all modules are connected with a flexible high-performance fabric.
%, each of which runs untrusted serverless users' code. 
The \emph{gateway service}, called MicroManager in AWS Lambda~\cite{agache:firecracker}, faces both the invocations for the function instances that run on this worker and the control path requests from the worker manager, e.g., to start and tear down function instances. 
To guarantee high security and deliver continuous worker-level monitoring, the gateway process mediates all the inbound and outbound traffic sent between front-end servers and function instances.
Upon the worker manager's requests, the gateway service interacts with the worker-local control plane, i.e., the host \textit{orchestrator}, that manages the resources of the worker. The host orchestrator processes the control plane requests of the gateway service by managing host resources, such as disk snapshots and virtual network interfaces, and interacts with per-instance \emph{shim} service on the host (\textit{oShim}). The shim service translates the high-level requests of the orchestrator into the low-level runtime API of the instances.
%\marios{ishim and oshim}

A function instance comprises a secure \emph{sandbox} that runs user's untrusted code of the function. To date, most leading serverless players choose virtualization-based sandboxes, e.g., a regular VM with a guest OS~\cite{agache:firecracker} or emulate guest OS environment~\cite{google:gvisor}, to deliver high security and isolation in the multi-tenant environment of a serverless worker.
During an instance's lifetime, the instance maintains a long-living connection with both the host orchestrator's shim service, by running a guest-based shim process (\textit{iShim}) that manages the sandbox environment, and a long-living data-plane connection to the gateway service of the worker. The function's code, provided by the developer of a serverless application, is injected into a software server, written in the programming language of the function, that processes the function's invocations \boris{- this sentence  is too complex. Does is matter for this paper that the SW server is written in the language of hte function? If it matters, explain why. if not, drop it.}. This server is able to process individual function invocations as well as a stream of independent invocations, albeit one at a time for security reasons.
\dmitrii{need to back up the server-in-language sandbox or say that it's one way of doing it}

\boris{The description in this section is a bit hard to follow. Do you need all of it? One potential way to make it easier to read is by following a request through the different layers of the system in a figure annotated with steps. That way, you can introduce the entities in the context of consecutive actions on a request, which is much more intuitive than just reading about a bunch of entities.}

\dmitrii{todo, move iShim and oShim to \ref{sec:containerd101}}

\begin{comment}

\textbf{Requirements}: flexible management of host resources, fast startup, performance and utilization metrics => plug-n-play software-based infrastructure\\

Gateway API that processes incoming triggers (e.g., HTTP requests)\\

Cluster scheduler that manages function instances across the server fleet\\

Host orchestrator (Containerd~\cite{containerd:industry}, Kata Containers~\cite{kata:containers}): maintains the lifecycle of all instances deployed on that host, manages the resources for function instances, incl. disk images, CPU and memory allocation.

Gateway process (called MicroManager in AWS~\cite{agache:firecracker}) that:
\begin{itemize}
    \item mediates all requests from the cluster scheduler, incoming requests (from triggers) and responses
    \item Interacts with the cluster scheduler and the host orchestrator\\
\end{itemize}


Each instance:
\begin{itemize}
    \item Function's code runs inside a VM.
    \item Externally VM is managed by an individual shim process in the host.
    \item Internally VM is managed by an pre-booted agent process (e.g., it mounts a disk snapshot as a virtual disk), connected via ttrpc/gRPC protocol to the host gateway process.\\
\end{itemize}

User-provided code is wrapped in an RPC-level fabric~\cite{agache:firecracker}, like gRPC~\cite{google:grpc} or Thrift~\cite{apache:thrift}, implying that the provider's server runs a user-provided handler written in a user-chosen high-level language.

\end{comment}



\subsection{Open-Source Benchmarking  for Serverless Systems and Architectural Research}

\boris{Would be good to explicitly state that (a) there is no open-source serverless infrastructure for at-scale experiments, and (b) the infrastructure used in existing work is incomplete/simplified. Not sure where to do it, but perhaps right in this section.}

The datacenter-scale architecture of serverless systems makes it imperative to carefully consider and model all the components of the distributed serverless infrastructure. Serverless research infrastructure needs to meet a number of key requirements that are representativeness in its architecture and each of the software components and the communication fabrics, robust evaluation methodology, and extensibility for fast prototyping of various research ideas. 

We present a complete end-to-end open-source infrastructure for serverless that achieves all of the aforementioned goals by building around the de facto standard plugin-based containerd framework~\cite{containerd:industry} for host orchestration, leveraging available industrial standard components and fabrics (including the Firecracker hypervisor~\cite{agache:firecracker} and gRPC communication framework~\cite{google:grpc}) while re-using and packaging functions from the state-of-the-art serverless function benchmark suite~\cite{kim:functionbench,kim:practical}. 

The infrastructure comprises loosely coupled modules for each of the essential components of the serverless architecture, seeking to enable innovation in any of these components with careful evaluation of the chosen components' implications on the end-to-end serverless system performance. All standard components are available as public forks of the industry and open-source community maintained repositories to allow seemless upgrades to the state-of-the-art continuously released features.

\marios{Think of adding a second figure with the components we used; reinforce the coordinator contribution}
The \textbf{centralized experiment coordinator service} implements load and latency measurement methodology. We build this custom component to drive all other infrastructure components through experiment phases, such as initial configuration and deployment of the distributed components, overall system warm-up phase, and stepping through a number of measurement phases (e.g., sweeping the load traffic, memory pressure, etc.). The components are coordinated via low latency gRPC fabric that allows fine-grain sub-millisecond coordination.
The coordinator also plays the role of the simplified worker manager, setting up long-living connections between the front-end and the workers. In future, we plan to delegate the worker manager's role to Kubernetes~\cite{k8s}, which is a de facto industry-standard cluster orchestrator.

\textbf{Front-end} is represented by a configurable number of custom load and latency clients that drive the invocation traffic and measure the end-to-end response latency of the deployed functions. 
Each load client drives its fraction of the load in an open loop, issuing invocation requests to functions according to functions popularity distribution (e.g., to model hot and cold functions as in a realistic deployment~\cite{shahrad:serverless}) and the target load. The latency clients issue one invocation request at a time, waiting for its completion, to exclude client-side queueing effects. Clients periodically report their throughput and latency measurements to the coordinator that aggregates the measured results.

The \textbf{ worker orchestration framework} includes containerd for managing function instances and the custom-build gateway service that mediates both the control and data plane inbound and outbound requests. 
We choose containerd because of its modularity, as nearly all containerd components are independent plugins, and wide support of the open-source and industrial communities led by Cloud Native Computing Foundation ~\cite{cncf,kata:containers,fc-ctrd:deep-dive,ctrd:gvisor}. This infrastructure supports different types of sandboxes, including virtual machines~\cite{agache:firecracker,kata:containers} and containers~\cite{opencontainers}, and common container toolchains. The supported toolchains provide a wide range of container primitives for deployment (e.g., container image layers), function instances isolation (e.g., network and filesystem namespaces along with system call whitelisting), host resources management (including network, CPU and memory limits per container), as well as logging and monitoring~\cite{prometheus}. 
We adopt the public containerd fork~\cite{fc-ctrd:github}, that is maintained by Amazon Firecracker engineers, that includes firecracker-specific shim components, both external and internal to the instance's sandbox. We showcase the flexibility of containerd by extending the original fork with the latest Firecracker feature that is virtual machine snapshots~\cite{fc:snaps} \boris{This is confusing. You have an official Amazon fork of Firecracker and you say you extend the fork with a Firecracker feature -- but why is that feature not in your fork?}.
%Amazon Firecracker~\cite{agache:firecracker}, Google gVisor~\cite{google:gvisor}), cluster orchestrators (e.g., Kubernetes~\cite{k8s}), and standard Open Container Initiative images~\cite{opencontainers}. 

For \textbf{sandbox} we choose Amazon Firecracker~\cite{agache:firecracker} that powers up Amazon Lambda and Fargate services but is widely adopted by other cloud providers, including Baidu AI Cloud~\cite{baidu:kata}, OpenNebula~\cite{opennebula:firework}, and WeaveWorks~\cite{weave:firekube}. A Firecracker sandbox is a full-blown virtual machine that runs a minimalist Linux kernel that delivers high security and isolation while providing performance close to container-based solutions.

\textbf{Gateway service} is implemented as a custom scalable multi-threaded gRPC-based software service that mediates both the control plane and data plane requests. We design the gateway service as a seamless extension of containerd that communicates to other components -- namely the coordinator, clients, containerd, and the function instances -- using the gRPC fabric that is the default choice for the existing containerd components.

\input{floats/tbl_functionbench}

\textbf{Functions} are implemented as gRPC-based single-threaded servers that run inside their corresponding sandboxes \boris{Need to explain/justify the single-thread aspect. Reviewers that are not knowledgable might think that vHive is not sufficiently 'serious' because it doesn't support multi-threading.}. The current release of vHive includes a simple \texttt{helloworld} function and eight functions from FunctionBench~\cite{kim:functionbench,kim:practical}, a representative suite of serverless functions written in Python that includes web processing, cryptography, image processing, machine learning models serving and training (Table~\ref{tbl:functionbench}). 
%a minimal helloworld function, web rendering, text encryption, image transformation, JSON serialization and de-serialization, three ML serving functions of different classes and frameworks, and client review predictor training (Table~\ref{tbl:functionbench}). 
FunctionBench originally distributes its benchmarks as collections of Python scripts; we wrapped these into gRPC servers deployed on top of Linux Alpine and containerized them into Docker/OCI images. \boris{I rewrote the last sentence - please check.}
%where each image comprises the function code packaged on top of Linux Alpine distribution. 


%>>>>>>>>>>>>>>>>>>>
\begin{comment}

\subsubsection{Requirements for a systems research platform}
\begin{itemize}
    \item Representativeness: Architecture and operation that are similar to those of industrial leaders, including both control and data planes, production-grade components and protocols, host and guest resources management, and virtualization (\S\ref{sec:serverless101}).
    \item End-to-end distributed system evaluation: robust methodology with high load and latency clients that drive the load towards both the control and data plane.
    \item Flexible and fast prototyping: plugin-based architecture based on industry-standard and industry-leading software components (containerd, gRPC), extensive test coverage.
\end{itemize}

\textbf{Load and latency clients as Front-end.} Open-loop load clients and close-loop latency clients based on gRPC~\cite{google:grpc}. Data path connects to the Gateway service. 

\textbf{Cluster scheduling.} TBD: our infra is compliant but right now it does not have cluster scheduling components. Long-term goal is to integrate our custom gateway service (see below) with containerd-cri plugin that would make it compatible with Kubernetes.

\textbf{Gateway service.} Custom Golang-based high-performance service that acts as a gRPC-level software router and a function instances manager via commands to the host orchestrator. Acts as a bridge between the universe of functions and and function instances. 
%Can be both stand-alone and co-located with each worker.

\textbf{Containerd as host orchestrator.} OCI and CRI/Kubernetes compliant, support for various sandboxes (runtimes), metrics collection with Prometheus. Support for overlay-based disk snapshots, virtual network configuration (incl., CNI), per-VM external and internal shim processes, connected with gRPC (ttrpc between the shims).

\textbf{Sandbox.} We chose Firecracker hypervisor as one of the leading solutions, used by AWS, Alibaba Cloud, Baidu AI Cloud~\cite{baidu:kata}, OpenNebula~\cite{opennebula:firework}, WeaveWorks~\cite{weave:firekube}. The sandbox runs a minimal Linux kernel

\textbf{Function server.} Deployed as an OCI-compliant container image that containerd supplies to the guest OS as a virtual disk to be mounted during guest OS boot process. The image comprises a gRPC server that wraps a user-provided function in a user-chosen language to serve RPCs that come from the clients (i.e., the Front-end fleet) via the Gateway service.

\textbf{Workloads aka Functions.} We adopt eight functions, from FunctionBench~\cite{kim:functionbench,kim:practical}, that cover a wide range of serverless use cases: image rotation, web rendering, encryption, json serialization, various ML serving and training. We integrate all workloads with a Python gRPC server. Functions are deployed in Alpine Linux images, commonly used in Serverless and Edge deployments due to its security and image-size advantages~\cite{alpine:containers}.

\end{comment}
%<<<<<<<<<<<<<<<<<<<<<<<<<<<<<





==> 5-methodology.tex <==

%\section{Methodology}
\section{Evaluation}
\label{sec:eval}

\cor{
In this section, we describe the platform setup, including the host and the guest setups, and present REAP evaluation results. In our experiments, we follow the methodology that is described in \S\ref{sec:char_method}, unless specified otherwise.
}

\subsection{Evaluation Platform}
\label{sec:method}
%\marios{Consider adding a sentence here to describe what is this methodology for}
%\marios{Consider moving this section as part of 4? This is the methodology used for these experiments, too, right?}
%%%\subsection{Serverless Host Infrastructure}

%\input{floats/worker_dia}

%%%\cor{We use vHive framework to set up a single worker server to be representative of the Amazon Lambda's proprietary MicroManager~\cite{agache:firecracker}. The vHive-CRI orchestrator interacts both with the control plane, i.e., Containerd, and acts as a software router that routes the function invocation requests, over the gRPC-based persistent connections~\cite{google:grpc}, to the appropriate instances and returns their responses. The vHive-CRI orchestrator establishes a persistent connection with Containerd that manages the lifecycle of all instances, starting or loading them from a snapshot on demand.}

%%%A function instance comprises a Firecracker MicroVM that runs a gRPC server running on top of Alpine Linux, \cor{except \texttt{video\_processing} that runs atop of Debian due to a problem with OpenCV installation on Alpine Linux}. Upon receiving an invocation, the gRPC server invokes a user-provided function and sends the function's response back to the vHive-CRI orchestrator.

\begin{comment} SUBMITTED VERSION BELOW
Our host infrastructure is based on the industry-standard Containerd framework~\cite{cncf,kata:containers,containerd:industry,ctrd:gvisor,fc-ctrd:deep-dive} that we extend to support the newly introduced Firecracker snapshots functionality~\cite{fc:snaps}. 
%Fig.~\ref{fig:infra} shows the overview of our infrastructure.
%We choose Containerd because of its modularity, as nearly all containerd components are independent plugins, and wide support of the open-source and industrial communities led by Cloud Native Computing Foundation ~\cite{cncf,kata:containers,fc-ctrd:deep-dive,ctrd:gvisor}.
%\boris{This next sentence is 8 lines and is absolutely impossible to parse. Please split into 2 or more sentences.} 
We introduce a custom-build host orchestrator, which is conceptually similar to Amazon Lambda's proprietary MicroManager~\cite{agache:firecracker}. The orchestrator interacts both with control plane, i.e., Containerd, and acts as a software router that routes the function invocation requests, over the gRPC-based persistent connections~\cite{google:grpc}, to the appropriate instances and returns their responses. 
The vHive-CRI orchestrator establishes a persistent connection with Containerd that manages the lifecycle of all instances, starting or loading them from a snapshot on demand. %Finally, the orchestrator maintains persistent connections with each active function instance. 
%Upon the orchestrator's requests, Containerd manages the lifecycle of all instances, starting or loading them from a snapshot on demand.
%The host orchestrator establishes a persistent connection with Containerd for control messages and persistent connections with each active function instance. 
%We use gRPC fabric~\cite{google:grpc} as a common choice for a general-purpose communication framework for communicating to Containerd and all function instances.

A function instance comprises a Firecracker MicroVM that runs a Containerd internal shim agent and a gRPC server running on top of Alpine Linux, \cor{except \texttt{video\_processing} that runs atop of Debian due to a problem with OpenCV installation on Alpine Linux}. Upon receiving an invocation, the gRPC server invokes a user-provided function and sends the function's response back to the orchestrator.
\end{comment}

%%%%MOVED to 5.2 We use a collection of benchmarks (\Table~\ref{tbl:functionbench}) and measure end-to-end cold-start latency. The latency includes all communication and processing steps, starting from issuing invocation requests to the host orchestrator that loads the appropriate function instances on demand and, once loaded, forwards the requests to these instances. At the end of execution, the instances send the responses, via the orchestrator, back to the benchmark. 
%\boris{The last paragraph of 5.2 also describes this latency measurement. I think you should move this paragraph to 5.2 and merge. You can then drop the first few sentences of this paragraph, thus saving space and avoiding redundancy.}

%issues both the control messages (i.e., function instances lifecycle) that go through the Containerd's chain of components and the data plane (i.e., function invocations) to the instances and collects their corresponding responses. When a gateway service injects 

%This infrastructure supports different types of sandboxes, including virtual machines~\cite{agache:firecracker,kata:containers} and containers~\cite{opencontainers}, and common container toolchains. The supported toolchains provide a wide range of container primitives for deployment (e.g., container image layers), function instances isolation (e.g., network and filesystem namespaces along with system call whitelisting), host resources management (including network, CPU and memory limits per container), as well as logging and monitoring~\cite{prometheus}. We adopt the public containerd fork~\cite{fc-ctrd:github}, that is maintained by Amazon Firecracker engineers, that includes firecracker-specific shim components, both external and internal to the instance's sandbox. We showcase the flexibility of containerd by extending the original fork with the latest Firecracker feature that is virtual machine snapshots~\cite{fc:snaps} \boris{This is confusing. You have an official Amazon fork of Firecracker and you say you extend the fork with a Firecracker feature -- but why is that feature not in your fork?}.
%Amazon Firecracker~\cite{agache:firecracker}, Google gVisor~\cite{google:gvisor}), cluster orchestrators (e.g., Kubernetes~\cite{k8s}), and standard Open Container Initiative images~\cite{opencontainers}. 

%For \textbf{sandbox} we choose Amazon Firecracker~\cite{agache:firecracker} that powers up Amazon Lambda and Fargate services but is widely adopted by other cloud providers, including Baidu AI Cloud~\cite{baidu:kata}, OpenNebula~\cite{opennebula:firework}, and WeaveWorks~\cite{weave:firekube}. A Firecracker sandbox is a full-blown virtual machine that runs a minimalist Linux kernel that delivers high security and isolation while providing performance close to container-based solutions.

%\textbf{Gateway service} is implemented as a custom scalable multi-threaded gRPC-based software service that mediates both the control plane and data plane requests. We design the gateway service as a seamless extension of containerd that communicates to other components -- namely the coordinator, clients, containerd, and the function instances -- using the gRPC fabric that is the default choice for the existing containerd components.



%\textbf{Functions} are implemented as gRPC-based single-threaded servers that run inside their corresponding sandboxes \boris{Need to explain/justify the single-thread aspect. Reviewers that are not knowledgable might think that vHive is not sufficiently 'serious' because it doesn't support multi-threading.}. The current release of vHive includes a simple \texttt{helloworld} function and eight functions from FunctionBench~\cite{kim:functionbench,kim:practical}, a representative suite of serverless functions written in Python that includes web processing, cryptography, image processing, machine learning models serving and training (Table~\ref{tbl:functionbench}). 
%a minimal helloworld function, web rendering, text encryption, image transformation, JSON serialization and de-serialization, three ML serving functions of different classes and frameworks, and client review predictor training (Table~\ref{tbl:functionbench}). 
%FunctionBench originally distributes its benchmarks as collections of Python scripts; we wrapped these into gRPC servers deployed on top of Linux Alpine and containerized them into Docker/OCI images. \boris{I rewrote the last sentence - please check.}


%\subsection{Evaluation Platform}

We conduct our experiments on a 2$\times$24-core Intel Xeon E5-2680 v3, 256GB RAM, Intel 200GB SATA3 SSD, running Ubuntu 18.04 Linux with kernel 4.15. We fix the CPU frequency at 2.5GHz to enable predictable and reproducible latency measurements. We disallow memory sharing among all function instances and disable swapping to disk, as suggested by AWS Lambda production guidelines~\cite{agache:firecracker,aws:prod}. 

We use a collection of nine Python-based functions (Table~\ref{tbl:functionbench})
\cor{from the representative FunctionBench~\cite{kim:functionbench,kim:practical} suite.\footnote{We omitted the microbenchmarks, MapReduce and Feature Generation because they require a distributed coordinator, and Video Face Detection that is not open source.}}
%. Nine of the studied functions are from the representative FunctionBench~\cite{kim:functionbench,kim:practical} suite. 
%The functions we selected cover diverse application domains and frameworks, and their runtime falls in the 1ms-10sec execution time range to match production deployments as reported for Azure Functions~\cite{shahrad:serverless}). Opportunity for \tac{} was {\em not} a criterion for function selection.
%, covering a wide range of application domains and frameworks. 
%\boris{Is this the entire FunctionBench suite or is it a subset? If subset, need to explain why and how these were chosen.} 
We also evaluate a simple \texttt{helloworld} function. 
The root filesystems for all functions are generated automatically by Containerd, using Linux device mapper functionality as used by Docker~\cite{docker:devmapper}, from Linux Alpine OCI (Docker) images.\footnote{\cor{The only exception is \texttt{video\_processing} that uses a Debian image due to a problem with OpenCV installation on Alpine Linux.}} 
\cor{Functions with large inputs (namely \texttt{image\_rotate}, \texttt{json\_serdes}, \texttt{lr\_training}, 
\texttt{video\_processing}) retrieve their inputs from an S3 server~\cite{minio} deployed on the same host.}
%We package function inputs (files, images, machine learning models, etc.) inside the OCI images, and use different inputs in the record and prefetch phases of {\tac}.

We optimize virtual machines for minimum cold-start delays, similar to a production serverless setup, as in \cite{agache:firecracker,kaffes:centralized}. The VMs run a guest OS kernel 4.14 without modules. Each VM instance has a single vCPU. We boot VM instances with 256MB guest memory, which is the minimum amount to boot all the functions in our study.


%\boris{minimum for the bulk of the functions doesn't sound sufficient for all functions. Please clarify.}
 


\input{floats/tbl_functionbench}


%In all experiments, we report end-to-end cold-start latency that includes all communication and processing steps, starting from issuing invocation requests to the vHive-CRI orchestrator that loads the appropriate function instances on demand and, once loaded, forwards the requests to these instances. At the end of execution, the instances send the responses, via the orchestrator, back to the benchmark. The latency includes both the control-plane delays (including interactions with Containerd and Firecracker hypervisor) and data-plane processing time that is gRPC requests processing and actual function execution. To simulate the low invocation frequency of serverless functions in production~\cite{shahrad:serverless}, we flush the host OS' page cache before each invocation of a cold function. We instrument the vHive-CRI orchestrator to break down the measured end-to-end latencies for various configurations that we evaluate.


%, which interacts with Containerd-based control plane and acts as a software router for sending requests to and from function instances,

%\dmitrii{highlight that the baseline Firecracker snaphots is equivalent to the cold-start Catalyzer config due to lazy paging. We don't consider other Catalyzer option because memory sharing is commonly disallowed in production environment}






==> Makefile <==
PAPER=ms
BIBCLOUDDIR=./bibcloud

all: $(PAPER).pdf

clean:
	rm -f $(PAPER).pdf prepress.pdf *.aux *.fdb_latexmk *.log *.bbl *.blg \
		*~ *.dvi *.vrb *.nav *.snm texput.* *.synctex.gz
	latexmk -C $(PAPER).tex

bib: 
	python $(BIBCLOUDDIR)/bibcloud.py $(PAPER)
	bibtex $(PAPER)

$(PAPER).pdf:
	latexmk -pdf \
		-latexoption=-file-line-error \
		-latexoption=-synctex=1 $(PAPER).tex \
		&& touch $(PAPER).dvi || ! rm -f $@
	#latexmk -pdf -latexoption=-halt-on-error \



#PAPER = asplos21-paper-template
#ABSTRACT = asplos21-extended-abstract-template
#TEX = $(wildcard *.tex)
#BIB = references.bib
#FIGS = $(wildcard figures/*.pdf figures/*.png graphs/*.pdf graphs/*.png)
#
#.PHONY: all clean
#
#all: $(PAPER).pdf $(ABSTRACT).pdf
#
#$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) jpaper.cls
#	echo $(FIGS)
#	pdflatex $(PAPER)
#	bibtex $(PAPER)
#	pdflatex $(PAPER)
#	pdflatex $(PAPER)
#
#$(ABSTRACT).pdf: $(TEX) $(BIB) $(FIGS) jpaper.cls
#	pdflatex $(ABSTRACT)
#	bibtex $(ABSTRACT)
#	bibtex $(ABSTRACT)
#	pdflatex $(ABSTRACT)
#	pdflatex $(ABSTRACT)
#
#
#clean:
#	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf $(ABSTRACT).pdf
#


==> artifact-eval.tex <==
\appendix
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

This artifact contains the source code of the vHive-CRI host orchestrator and includes the necessary binary files of its dependencies, namely Firecracker-Containerd shim binaries, Firecracker hypervisor and jailer, default rootfs for Firecracker MicroVMs, MinIO object store server, and client binaries. 
The reviewers require Ubuntu 18.04 with root access and hardware virtualization support (e.g., VT-x), a platform with the root partition mounted on an SSD is preferred.
The artifact lists the instructions to reproduce Fig.~\ref{fig:eval_one_instance} for the configuration that uses vanilla Firecracker snapshots and the configuration that uses {\tac}-based snapshots. The reviewers can run functions from the representative FunctionBench suite, using pre-built Docker images.

\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
  \item {\bf Algorithm: Record and prefetch a serverless function's memory footprint from a VM snapshot}
  \item {\bf Program: the vHive-CRI orchestrator, using Firecracker snapshots and {\tac}-accelerated snapshots}
  \item {\bf Compilation: GCC 7, Golang 1.14 (installed by the provided scripts)}
  \item {\bf Binary: Firecracker hypervisor (x86, 64-bit), Containerd binaries  (x86, 64-bit), default rootfs image for a VM, MinIO server and client}
  \item {\bf Data set: Dockerized functions from FunctionBench; few functions include food reviews, photos, videos (all included)}
  \item {\bf Run-time environment: Ubuntu 18.04, kernel v4.15, root access is required}
  \item {\bf Hardware: Intel or AMD x86 CPU with hardware virtualization (VT-x for Intel or AMD-V for AMD) support and KVM, recommended but not required to mount the root partition on an SSD}
  \item {\bf Metrics: Function cold-start delay, milliseconds}
  \item {\bf Output: Text files}
  \item {\bf Experiments: Cold start delays measurement}
  \item {\bf How much disk space required (approximately)?: At least 20GB mounted for the root partition "/"}
  \item {\bf How much time is needed to prepare workflow (approximately)?: 10 minutes}
  \item {\bf How much time is needed to complete experiments (approximately)?: 1 hour}
  \item {\bf Publicly available?: yes}
  \item {\bf Code licenses: MIT, Apache 2.0}
  \item {\bf Data licenses: CC0 1.0 Universal (CC0 1.0)
Public Domain Dedication for reviews, The Pexels License for photos, royalty-free videos from \url{sample-videos.com} }
  \item {\bf Archived (provide DOI)?: 10.5281/zenodo.4321807, may be updated after artifact evaluation}
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\textbf{Clean bare-metal setup is available.} Upon a request from the reviewers, we can provide a bare-metal access to a clean Ubuntu 18.04 machine on CloudLab (\url{https://www.cloudlab.us}) that meets all the hardware and software requirements. The reviewers may indicate their need in the comments to the submission on the submission HotCRP website or by email to \url{dmitrii.ustiugov@ed.ac.uk}. The reviewers would then need to create their account on CloudLab, upload their SSH keys to CloudLab, then ask to join the project, called \texttt{RPerf}. Once we approve this request, the reviewers would be able to \texttt{ssh} to the machine (we would provide the exact URL of the machine) with a command like the following:

\begin{verbatim}
ssh -p 22 username@hpXXX.utah.cloudlab.us
\end{verbatim}

The reviewers are free to use any other machine if they choose so.

\subsubsection{How to access}

The code can be pulled from the public Git repository that is available by \url{https://github.com/ease-lab/vhive}, where the branch \texttt{minio-ip-parameter} is prepared for artifact evaluation. The required project dependencies are available by \url{https://github.com/ease-lab/firecracker-containerd}, \url{https://github.com/ease-lab/firecracker}, and \url{https://github.com/ease-lab/firecracker-go-sdk}. The provided scripts install and set up all the dependencies and downloads all binaries, requiring no action from the reviewer.


\subsubsection{Hardware dependencies}
The artifact evaluation procedure requires an x86 CPU, Intel or AMD, with hardware virtualization support (VT-x for Intel or AMD-V for AMD). The root partition is recommended to be mounted on an SSD, however no issues are expected if the partition is mounted on an HDD. However, with an HDD, {\tac} provides higher speed-up over the vanilla Firecracker snapshots than shown in Fig.~\ref{fig:eval_one_instance}.


\subsubsection{Software dependencies}

The recommended OS setup is Ubuntu 18.04 with kernel v4.15.  The root partition must have at least 20GB available. The setup scripts execute commands with \texttt{sudo} so the system must allow executing commands with \texttt{sudo} without asking for the password (i.e., requires to set up passwordless \texttt{sudo}). Also, KVM must be available (for example, executing in a virtual machine is only possible if KVM is exposed).

To check if the machine has KVM available, type:

\begin{verbatim}
[ -r /dev/kvm ] && [ -w /dev/kvm ] && \
echo "KVM is available" || echo "KVM is unavailable"
\end{verbatim}

If KVM is unavailable but the machine has VT-x or AMD-V support, run the following command:

\begin{verbatim}
sudo setfacl -m u:${USER}:rw /dev/kvm
\end{verbatim}

\subsubsection{Data sets}
All the necessary datasets for the functions are provided inside Docker images or stored in the Git repository. The provided scripts provide access to all of these datasets so that no action is required from the reviewer.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

To fetch the repository:
\begin{verbatim}
git clone https://github.com/ease-lab/vhive.git \
--branch minio-ip-parameter
\end{verbatim}

To install the necessary packages and set up the machine for the experiments, run the following command from a non-root user (the user must be allowed to run commands with `sudo`) from the root folder of the repository (\texttt{./vhive}):
\begin{verbatim}
./ae_scripts/setup.sh
\end{verbatim}

Note that the script is safe to run several times, e.g., if the previous run was interrupted, albeit it may show you that MinIO bucket already exists, which is not a problem.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

First, run the experiment to collect the cold start delays for all the functions from Fig.~\ref{fig:eval_one_instance}) with the configuration with vanilla Firecracker snapshots:
\begin{verbatim}
./ae_scripts/run_all.sh baseline
\end{verbatim}

If you use CloudLab or if you have a machine with the root partition with less than 40GB, please reboot the machine. The reboot is necessary to free up the storage space on the root partition after de-allocating Docker images due to the use of the device mapper by Firecracker-Containerd. The issue is known but is not yet fixed in the upstream repository (\url{https://github.com/moby/moby/issues/3182#issuecomment-228298975}).

Once the machine is online again, please repeat the experiment with the configuration with {\tac} snapshots:
\begin{verbatim}
./ae_scripts/run_all.sh reap
\end{verbatim}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected result}

The per-function average latencies (averaged across 5 cold starts of each function) for both configurations are written to a CSV file that can be printed to the console (from the repository's root folder):
\begin{verbatim}
cat all_results/results.csv
\end{verbatim}

Each line of this CSV file contains three comma-separated fields: the function name, the mode (baseline or reap), and the average cold start delay in milliseconds.
The CSV file is appended with a new line after each function is evaluated so do not delete this file before both experiments are finished. 
%There could be sporadic issues that may need re-running some of the functions. 
%Please see \S\ref{sec:notes} that details the known issues and possible fixes or workarounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}
\label{sec:customization}

The workflow allows to specify the subset of functions to be run in an experiment. The functions are listed in \texttt{./ae\_scripts/functions.txt}, which is the relative path to the repository's root folder. By default, the file contains all the functions that are listed in Table~\ref{tbl:functionbench} but the reviewers can delete (not comment out) some of the functions from the file to repeat the experiment only for a subset of functions. This can be useful if an experiment is interrupted or failed due to some reason.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}
\label{sec:notes}

%The CSV file with the results is appended with a new line after each function is evaluated so one should not delete the file before both experiments are finished. 
There could be sporadic issues that may need re-running some of the functions (see the instructions for re-running in \S\ref{sec:customization}):

\begin{itemize}
    \item The root partition is full. Need to reboot the machine so that the storage gets free from the device-mapper disk images.
    \item The problem may be related to an I/O timeout. In this case, the corresponding error message could be inspected in\\ \texttt{./all\_results/$<$mode$>$/$<$function$>$/test.out} file. The error is sporadic so re-running the necessary subset of functions would be enough.
\end{itemize}

In case of any issue during the experiments, please create a tarball of the results folder, and send it to us via HotCRP or by email \texttt{dmitrii.ustiugov@ed.ac.uk}, with a command (that must be run from the repository's root folder) for further troubleshooting:

\begin{verbatim}
tar -zcvf results.tar.gz all_results
\end{verbatim}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}

Submission, reviewing and badging methodology:

\begin{itemize}
  \item \url{https://www.acm.org/publications/policies/artifact-review-badging}
  \item \url{http://cTuning.org/ae/submission-20201122.html}
  \item \url{http://cTuning.org/ae/reviewing-20201122.html}
\end{itemize}
}

==> bibcloud/.git/objects/26/25753ecb8adce4ffbca8b6893f72d551446d97 <==
x¥ÎQjÃ0Ð~ëû_+©',(%rÕî*68–q¤û×4Gó÷†áöx,\LýP…HŒÊ–Dªè´Xσ«!¸¦3©˜Ý:LT%Ÿ*GB™£µõ¬RmNê&ï•>·nÒ¿ã¾-mƒo}Á¥¼àª{]/<ÿ€
9Å)"¯Ÿè
ÿ_íúֈ)Káµ
úE™ÆS¡U²îÀ3mw5»¼WQ

==> bibcloud/dcsl-latex.tex <==


 
% this file is compatible with 
%  - the sigplanconf.sty 
%  - the SIG-ALT-FULL.CLS - VERSION 1.6
%  - also the USENIX conferences (osdi, etc)
%  - also ASPLOS (jpaper)

% v0.1 - 2018-06-20


% Comment/comment the lines to dynamically configure the file

\newif\ifcomments
%\commentstrue



% PACKAGES THAT MUST ALWAYS BE DEFINED ONE WAY OR ANOTHER

\usepackage{xspace}                         % auto-space mgmt for commands
\usepackage{subfig}                         % subfloat
\usepackage[normalem]{ulem}                 % sout
\usepackage{upgreek}
\usepackage{comment}                        % \begin{comment}
\usepackage{rotating}
\usepackage{graphicx}
\usepackage{multirow}


%USENIX conferences are just {article} -- requires this additional:
%
\makeatletter
\@ifclassloaded{sigplanconf}{
%sigplanconf only additions
\usepackage{gensymb}  %socc - celsius
}{
%else
\usepackage{cite} % automatically sorts the citations.  there is an optional [nocompress].

\@ifclassloaded{jpaper}{
% ASPLOS papers
}{
% USENIX papers (in practice)
\usepackage{gensymb}  %socc - celsius
\usepackage[usenames, dvipsnames]{color}
\usepackage{url}
}
}
\makeatletter



%% poor man's layout
%% when \usepackage{layout} .... \layout is broken

\newcommand{\printlayout}{{\bf The textwidth \the\textwidth; the columnwidth is \the\columnwidth}}

% HYPHENATION HELP

\hyphenation{user-space}

% GENERIC THINGS

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\egparen}[1]{(\eg~#1)\xspace}
\newcommand{\ieparen}[1]{(\ie~#1)\xspace}
\newcommand{\egp}[1]{\egparen{#1}}
\newcommand{\iep}[1]{\ieparen{#1}}

\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\twiddle}{$\sim$}
\newcommand{\microsecond}{$\upmu{}$s\xspace}
\newcommand{\nanosecond}{$ns$\xspace}

\newcommand{\myitem}{\noindent$\bullet\hspace{10pt}$}
\newcommand{\myparagraph}[1]{\vspace{1em}\noindent {\bf #1:}}
 
%DCSL


\newcommand{\edb}[1]{\noindent{{\bf \fbox{EdB:} {\textcolor{red}{\it#1}}}}}
\newcommand{\george}[1]{\noindent{{\bf \fbox{GP:} {\textcolor{blue}{\it#1}}}}}
\newcommand{\marios}[1]{\noindent{{\bf \fbox{MK:} {\textcolor{green}{\it#1}}}}}
\newcommand{\jf}[1]{\noindent{{\bf \fbox{JF:} {\textcolor{Peach}{\it#1}}}}}
\newcommand{\ag}[1]{\noindent{{\bf \fbox{AG:} {\textcolor{Gray}{\it#1}}}}}
\newcommand{\sam}[1]{\noindent{{\bf \fbox{Sam:} {\textcolor{cyan}{\it#1}}}}}



%make sure to always define in the main latex file
%\newcommand{\system}{\textsc{FOOBAR}\xspace}


==> bibcloud_old/dcsl-latex.tex <==


 
% this file is compatible with 
%  - the sigplanconf.sty 
%  - the SIG-ALT-FULL.CLS - VERSION 1.6
%  - also the USENIX conferences (osdi, etc)
%  - also ASPLOS (jpaper)

% v0.1 - 2018-06-20


% Comment/comment the lines to dynamically configure the file

\newif\ifcomments
%\commentstrue



% PACKAGES THAT MUST ALWAYS BE DEFINED ONE WAY OR ANOTHER

\usepackage{xspace}                         % auto-space mgmt for commands
\usepackage{subfig}                         % subfloat
\usepackage[normalem]{ulem}                 % sout
\usepackage{upgreek}
\usepackage{comment}                        % \begin{comment}
\usepackage{rotating}
\usepackage{graphicx}
\usepackage{multirow}


%USENIX conferences are just {article} -- requires this additional:
%
\makeatletter
\@ifclassloaded{sigplanconf}{
%sigplanconf only additions
\usepackage{gensymb}  %socc - celsius
}{
%else
\usepackage{cite} % automatically sorts the citations.  there is an optional [nocompress].

\@ifclassloaded{jpaper}{
% ASPLOS papers
}{
% USENIX papers (in practice)
\usepackage{gensymb}  %socc - celsius
\usepackage[usenames, dvipsnames]{color}
\usepackage{url}
}
}
\makeatletter



%% poor man's layout
%% when \usepackage{layout} .... \layout is broken

\newcommand{\printlayout}{{\bf The textwidth \the\textwidth; the columnwidth is \the\columnwidth}}

% HYPHENATION HELP

\hyphenation{user-space}

% GENERIC THINGS

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\egparen}[1]{(\eg~#1)\xspace}
\newcommand{\ieparen}[1]{(\ie~#1)\xspace}
\newcommand{\egp}[1]{\egparen{#1}}
\newcommand{\iep}[1]{\ieparen{#1}}

\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\twiddle}{$\sim$}
\newcommand{\microsecond}{$\upmu{}$s\xspace}
\newcommand{\nanosecond}{$ns$\xspace}

\newcommand{\myitem}{\noindent$\bullet\hspace{10pt}$}
\newcommand{\myparagraph}[1]{\vspace{1em}\noindent {\bf #1:}}
 
%DCSL


\newcommand{\edb}[1]{\noindent{{\bf \fbox{EdB:} {\textcolor{red}{\it#1}}}}}
\newcommand{\george}[1]{\noindent{{\bf \fbox{GP:} {\textcolor{blue}{\it#1}}}}}
\newcommand{\marios}[1]{\noindent{{\bf \fbox{MK:} {\textcolor{green}{\it#1}}}}}
\newcommand{\jf}[1]{\noindent{{\bf \fbox{JF:} {\textcolor{Peach}{\it#1}}}}}
\newcommand{\ag}[1]{\noindent{{\bf \fbox{AG:} {\textcolor{Gray}{\it#1}}}}}
\newcommand{\sam}[1]{\noindent{{\bf \fbox{Sam:} {\textcolor{cyan}{\it#1}}}}}



%make sure to always define in the main latex file
%\newcommand{\system}{\textsc{FOOBAR}\xspace}


==> floats/design_prefetch.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth,trim={10cm 10cm 10cm 10cm},clip]{figs/design_prefetch.pdf}
\caption{{\tac} prefetch phase.}
\label{fig:design_prefetch}
\end{figure}

==> floats/eval_coldstart_per_sec.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.98\columnwidth]{figs/blank.png}
\caption{Microbenchmark: Cold-starts/sec per workload. ETA: 9.08}
\label{fig:cold_start_per_sec}
\end{figure}

==> floats/eval_e2e_mix.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.98\columnwidth]{figs/blank.png}
\caption{End-to-end lat/throughput for workload mix (X\% cold-start ratio). Similar to Fig \ref{fig:char_e2e}. ETA 12.08}
\label{fig:e2e_mix}
\end{figure}

==> floats/eval_e2e_one.tex <==
\begin{figure}[t]
\centering
\subfloat[Wld 1 \textbf{ETA: 12.08}]{
    \includegraphics[width=0.98\columnwidth]{figs/blank.png}
    \label{fig:e2e_one_wld1}}
\newline
\centering

\centering
\subfloat[Wld 2 \textbf{ETA: 12.08}]{
    \includegraphics[width=0.98\columnwidth]{figs/blank.png}
    \label{fig:e2e_one_wld2}}
\newline

\centering
\subfloat[Wld 3 \textbf{ETA: 12.08}]{
    \includegraphics[width=0.98\columnwidth]{figs/blank.png}
    \label{fig:e2e_one_wld3}}
\newline




\caption{End-to-end Latency/throughput for each workload (X\% cold-start ratio).}
\label{fig:e2e_one}
\end{figure}

==> floats/fl_invoc_freq.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.98\columnwidth]{figs/azure_invoc_freq.png}
\caption{Serverless application, comprising 1 or more functions, invocation frequency CDF~\cite{shahrad:serverless}.}
\label{fig:azure_invoc_freq}
\end{figure}

==> floats/worker_dia.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figs/worker_dia.pdf}
\caption{Serverless host infrastructure overview
}
\label{fig:infra}
\end{figure}

==> old versions/3-characterization.tex <==

\section{Serverless Latency and Memory Footprint Characterization}
\label{sec:cold_lat_study}

Serverless providers aim to combine low cold-start time of the function instances and the efficient main memory utilization on the physical nodes that host function instances. 
%Agache et al. demonstrated that the cold-start latency is dominated by the host-based overheads as compared to the cluster infrastructure\cite{agache:firecracker}. 
In this section, we examine the cold-start latency and memory footprint and locality characteristics of function instances in our serverless framework, using the state-of-the-art Firecracker VM snapshotting feature~\cite{fc:snaps}.
\marios{I think we need to describe the experiments run or at least the functions used and where they come from.}
%Tradeoff: latency vs memory utilization (cost-efficiency). Corroborating the prior work, we find that the dominant serverless latency part resides on the hosting server, as cluster infrastructure, namely the scale-out front-end and scale-up high-throughput low-latency worker manager, is able to process requests in under 30ms~\cite{agache:firecracker}. 

\subsection{Cold-Start Latency and Memory Footprint Trade-off}
\label{sec:lat_mem_tradeoff}

\input{floats/char_lat}
\input{floats/char_footprint}

\boris{mention that we assume local storage for the snapshots, which is the best case latency wise}

When a function instance remains warm (i.e., stays in memory) after booting, the instance delivers the lowest possible response time latency (Fig.~\ref{fig:lat_warm}) but occupies hundreds of MBs of pricey memory (Fig.~\ref{fig:char_footprint}). As a result, the overall footprint of function instances may span to several hundreds of gigabytes, assuming that serverless providers co-locate thousands of different functions instances on the same host while disallowing memory sharing for security reasons~\cite{agache:firecracker}. 

First, we analyse the number of distinct guest-physical memory pages that a function instance accesses during processing an invocation request. 
%by loading function instances from a VM snapshot using Firecracker's snapshotting feature. 
After loading the VMM's and emulation devices' state from a snapshot is complete, the instance starts to process the invocation request, accessing the necessary subset of the guest memory that raises page faults to the guest-memory backing file in the host OS.
%, lazily bringing only a handful of pages from the guest memory file following the page faults. 
As guest-physical memory in Linux is a regular virtual memory region~\cite{bugnion:hardware}, we register the guest memory footprint reported by Linux \texttt{ps} utility, as a number of pages in the host's physical memory that are allocated for the VM, right after the gateway service receives a response from the function. We then compare the footprint of the function instances loaded from a snapshot to the footprint of the corresponding function instances that serves an invocation after they were booted. Fig.~\ref{fig:char_footprint} shows that functions' working sets span 8-34MB that is mere 4-13\% of the functions' memory footprint after booting. This discrepancy can be attributed to the fact that a function instance engages much more logic in the guest OS and user-defined initialization part of the functions during the boot time as compared to processing the actual function invocation request.


%that is between receiving the invocation request from the gateway process and sending the response back to the gateway process, as compared to the memory footprint reported by Linux \texttt{ps} utility after booting and initializing a fresh function instance. Firecracker hypervisor maps guest memory as a plain file so that the memory pages are brought in from the filesystem lazily upon guest accesses, revealing the function's working set of guest memory pages.We find that functions' working sets span 8-34MB that is mere 4-13\% of the functions' memory footprint after booting. This can be attributed to the fact that a function instance engages much more logic in the guest OS and user-defined initialization part of the functions during the boot time as compared to function invocation processing.

%Tracing guest page faults reveals\footnote{To trace guest memory accesses, we map and register a VM's guest memory as a virtual memory region for page faults handling by a userland process~\cite{man:userfaultfd}.} that the memory pages that a function instance accesses 

%To avoid memory waste, cloud vendors keep function instance alive for limited time, e.g., 10-20 minutes~\cite{shahrad:serverless,agache:firecracker}. However, boot latency can easily climb up to multiple seconds. For example, for the functions that we study, the cold-start time varies from 2.7 to 21.4 seconds. The functions' boot time is dominated by the VM boot time and mounting the virtual disk with the function OCI/docker image as well as the function's user-defined initialization that may include reading files or training an ML model.

%Emerging VM snapshotting mechanisms (\S\ref{sec:cold-start101}) like in Firecracker, 

Firecracker snapshotting maps the guest memory as a file-backed memory region relying on lazy paging that, as we find, comes at a significant overhead due to thousands of page faults that arise during a single invocation of a function.
%While VM snapshotting mechanisms eliminate the guest OS boot time and function initialization overheads that dominate the VM boot time~\cite{du:catalyzer}, these mechanisms' mapping of the guest memory file for lazy paging induces a significant overhead due to a large number of page faults.
%at the cost of adding moderate 50ms overhead for restoring the VMM state and the emulated network and block devices of the VM. However, 
Fig.~\ref{fig:lat_snap} shows that the time an instance spends in processing of an invocation request increases by one to two orders of magnitude as compared to the corresponding warm functions for the majority of the studied functions. Also, restoring the data path TCP connection from the gateway service to the function instance takes at least 130ms that alone makes up a significant overhead. 
\boris{Fig 3a and 3b should be merged. Use the log Y-axis. I assume the last sentence (restore TCP) is related to 'reconnect to function' in the graph. Make sure you use the same terminology in the graph and in the text. }
%These elevated overheads are related to the large number of page faults that guest memory accesses cause.

%VM snapshot/restore mechanisms allow to eliminate both of the sandbox boot and function initialization overheads. Fig shows...
%by loading the state of VMM, emulated devices, and mapping guest memory as a plain file. However, function processing time (user time) increases by up to two orders of magnitude with snapshot loading vs. warm function response. We find that the reason for this is the large number of page faults that functions experience after loading, as functions tend to have a relatively large memory footprint.


\subsection{Characterizing Functions' Spatial and Temporal Memory Locality}
\label{sec:mem_locality}


%%%% STOPPED HERE DMITRII To understand the source of the guest memory page faults, we study the spatial and 

Given the stateless nature of functions, user and guest kernel code pages account for a large fraction of functions' footprint. As explained in \S\ref{sec:containerd101}, providers deploy additional control-plane services (i.e., iShim in our case) inside a function's sandbox and use general-purpose communication fabric (i.e., gRPC in our case) to connect functions to the gateway service. The gRPC framework uses the standard TCP network protocol, similarly to AWS Lambda~\cite{agache:firecracker}, adding guest OS's networking stack to the footprint of a function instance. 
%Finally, the Firecracker hypervisor itself accounts for 3MB of memory footprint, 
We estimate the overall infrastructure tax to account for up to 8MB of a function's guest-memory footprint, which can be derived from the footprint of the \texttt{helloworld} function. Other functions exhibit larger memory footprints of up to 34MBs because these functions import more and larger libraries (e.g., Python modules for machine learning frameworks) or use larger input datasets (e.g., JSON files, images).

\input{floats/char_contig}

As the code accounts for a large fraction of the memory footprint, the guest OS allocates these pages randomly across the guest-physical memory, following address space layout randomization. We obtain the locations of these pages by augmenting the Firecracker hypervisor code to register the guest-physical memory region for page fault handling by a user-level monitor program. Using Linux \texttt{userfaultfd} feature~\cite{man:userfaultfd}, the monitor serves the page faults on behalf of the host OS as well as traces the virtual addresses, i.e., the guest-physical memory addresses, that triggered the faults.
Fig.~\ref{fig:char_contiguity} shows that the average length of the contiguous regions of the guest-physical memory is around two pages for all functions, except \texttt{image\_rotate} and \texttt{json\_serdes} that show contiguity of up to 4 pages. As a result, the pages are scattered across the guest-memory backing file inducing high page fault delays because sparse accesses to disk cannot benefit from the host OS's run-ahead prefetching. \boris{Why disk? I thought a function is either in memory or is loaded over a network if cold booted. I didn't see snapshots introduced (may be I missed it).}



%Spatial locality. A function's memory pages are scattered around guest physical memory due to the (guest) OS memory allocation mechanisms. Buddy allocator randomizes the placement of code pages that results in limited contiguity of of the function's pages inside the guest physical memory (Fig.~\ref{fig:char_contiguity}). As a result, functions' cold-start is dominated by many sparse accesses to disk, rendering disk run-ahead prefetch ineffective.

\input{floats/char_pages_reuse}

We identify that functions exhibit strong reuse patterns in accessing guest memory \textit{across} function invocations. First, the function-as-a-service programming paradigm encourages decomposition of the functions into special-purpose compact pieces of functionality, functions naturally reuse the bulk of the memory pages while processing different inputs. For example, when rotating different images or evaluating different customer reviews, functions use the same calls to the same libraries and rely on the same functionality inside the guest kernel, e.g., the networking stack. Second, the functions engage the same functionality that is a part of the provider's infrastructure (e.g., iShim). Finally, we observe that even when a function's code performs a dynamic allocation, the guest OS buddy allocator is likely to make the same or similar allocation decisions as its decisions are based on the state of its internal structures (i.e., lists of free memory regions) that are the same after loading from the same VM snapshot.
%be in exactly the same or similar state in each invocation provided that the function instance restores from the same VM snapshot. 
Fig.~\ref{fig:char_pages_reuse} demonstrates that most functions reuse more than 97\% of the memory pages. Only \texttt{image\_rotate} and \texttt{lr\_training} reuse slightly lower fraction of the data pages,  76\% and 72\% correspondingly, because these functions have relatively large inputs that are photos and training datasets of 4MB and 10MB sizes.
\\

To summarize, we identify that page faults to the guest-physical memory backing file dominate the cold-start latency of the serverless functions that we studied. These page faults trigger a large number of time-consuming sparse disk accesses to the guest memory file. However, our main insight is that functions reuse a large fraction of memory pages across invocations that provides an opportunity for prefetching of the guest memory pages from the disk into main memory before the VM requests them directly.
%dominated by page faults that become time-consuming as the guest memory pages accessed during a function's execution are scattered, translating to sparse accesses to disk. Our main insight is that functions reuse a large fraction of memory pages across invocations.


\begin{comment}

\subsection{Boot-based cold start.}
\label{sec:char_boot}

\subsection{Snapshot-based cold start.}
\label{sec:char_snap}



\textbf{Latency charts}: 
\begin{itemize}
    \item firecracker-containerd boot time breakdown => vdisk mount and language interpreter startup dominate (1 sec for each). 
    \item same with Firecracker snapshots. => page faults dominate (100s of ms)\\
\end{itemize}

%\input{floats/char_e2e}

%\dmitrii{TBD: lat/thru curve to show the capabilities of the infra. Uniform workload mix. Y axis: latency percentiles, X axis: throughput.}



\textbf{Memory footprint chart}: process vs. VM-after-boot vs. actually used => only 10-30\% of after boot memory is used upon invocation.\\



\textbf{Pages reuse chart.} 70+\% and 99\% of pages are the same for many functions. => can be considered as a working set

\textbf{Guest physical memory contiguity chart.} => Pages are sparse

\textbf{Insight}: a function's footprint is dominated by the code and guest OS code/state. Examples: network/virtio stack, gRPC and user libraries, kernel code. All these are reused across different invocations of the function.

\end{comment}


==> old versions/3-infra.tex <==
\section{End-to-End Serverless Infrastructure}
\label{sec:characterization}

\boris{Add a lead-in: we overview general serverless architecture, and describe our open-source infrastructure for at-scale serverless experimentation.}

\subsection{Serverless Architecture Overview}
\label{sec:containerd101}


Serverless systems have a datacenter-scale distributed architecture that comprises an extensive number of components and services (Fig.~\ref{fig:serverless_overview}). The software components are connected with a flexible REST API \boris{define REST} fabric that enables flexible management and resources usage monitoring while delivering high performance.


\input{floats/fl_serverless_overview}

\boris{Need to make it clear that you're describing a typical industry deployment, not something you cooked up. If you could say that the following is representative of AWS Lambda or Azure Functions, with a citation, that would be perfect.}
A serverless system comprises of the scale-out shared-nothing front-end fleet of servers facing the serverless function invocations, the worker fleet that executes the function code, and the worker manager that connects the two together~\cite{agache:firecracker,shahrad:serverless,krook:openwhisk}.
A function invocation, in a form of a REST API request, first arrives at one of the front-end servers for request authentication and mapping of the request to its corresponding function. 
%Then, the request may follow the slow \emph{control path}, e.g., when no instances of the function are running, or fast \emph{data path}. 

The \emph{worker manager} is a scale-up highly available service that maintains the mapping of the functions to their available instances and manages the fleet of worker servers that run the instances of the function. If no instances of the function are running, the worker manager selects a worker that can start a new instance of the function, based on the current load and available resources of the worker. To facilitate recurring events processing, the worker manager enables sticky routing connecting front-end servers to a minimal number of workers that allows reuse of the already running function instances.

Worker servers feature a highly modular architecture that aims to deliver high performance and security while running thousands of function instances, where all modules are connected with a flexible high-performance fabric.
%, each of which runs untrusted serverless users' code. 
The \emph{gateway service}, called MicroManager in AWS Lambda~\cite{agache:firecracker}, faces both the invocations for the function instances that run on this worker and the control path requests from the worker manager, e.g., to start and tear down function instances. 
To guarantee high security and deliver continuous worker-level monitoring, the gateway process mediates all the inbound and outbound traffic sent between front-end servers and function instances.
Upon the worker manager's requests, the gateway service interacts with the worker-local control plane, i.e., the host \textit{orchestrator}, that manages the resources of the worker. The host orchestrator processes the control plane requests of the gateway service by managing host resources, such as disk snapshots and virtual network interfaces, and interacts with per-instance \emph{shim} service on the host (\textit{oShim}). The shim service translates the high-level requests of the orchestrator into the low-level runtime API of the instances.
%\marios{ishim and oshim}

A function instance comprises a secure \emph{sandbox} that runs user's untrusted code of the function. To date, most leading serverless players choose virtualization-based sandboxes, e.g., a regular VM with a guest OS~\cite{agache:firecracker} or emulate guest OS environment~\cite{google:gvisor}, to deliver high security and isolation in the multi-tenant environment of a serverless worker.
During an instance's lifetime, the instance maintains a long-living connection with both the host orchestrator's shim service, by running a guest-based shim process (\textit{iShim}) that manages the sandbox environment, and a long-living data-plane connection to the gateway service of the worker. The function's code, provided by the developer of a serverless application, is injected into a software server, written in the programming language of the function, that processes the function's invocations \boris{- this sentence  is too complex. Does is matter for this paper that the SW server is written in the language of hte function? If it matters, explain why. if not, drop it.}. This server is able to process individual function invocations as well as a stream of independent invocations, albeit one at a time for security reasons.
\dmitrii{need to back up the server-in-language sandbox or say that it's one way of doing it}

\boris{The description in this section is a bit hard to follow. Do you need all of it? One potential way to make it easier to read is by following a request through the different layers of the system in a figure annotated with steps. That way, you can introduce the entities in the context of consecutive actions on a request, which is much more intuitive than just reading about a bunch of entities.}

\dmitrii{todo, move iShim and oShim to \ref{sec:containerd101}}

\begin{comment}

\textbf{Requirements}: flexible management of host resources, fast startup, performance and utilization metrics => plug-n-play software-based infrastructure\\

Gateway API that processes incoming triggers (e.g., HTTP requests)\\

Cluster scheduler that manages function instances across the server fleet\\

Host orchestrator (Containerd~\cite{containerd:industry}, Kata Containers~\cite{kata:containers}): maintains the lifecycle of all instances deployed on that host, manages the resources for function instances, incl. disk images, CPU and memory allocation.

Gateway process (called MicroManager in AWS~\cite{agache:firecracker}) that:
\begin{itemize}
    \item mediates all requests from the cluster scheduler, incoming requests (from triggers) and responses
    \item Interacts with the cluster scheduler and the host orchestrator\\
\end{itemize}


Each instance:
\begin{itemize}
    \item Function's code runs inside a VM.
    \item Externally VM is managed by an individual shim process in the host.
    \item Internally VM is managed by an pre-booted agent process (e.g., it mounts a disk snapshot as a virtual disk), connected via ttrpc/gRPC protocol to the host gateway process.\\
\end{itemize}

User-provided code is wrapped in an RPC-level fabric~\cite{agache:firecracker}, like gRPC~\cite{google:grpc} or Thrift~\cite{apache:thrift}, implying that the provider's server runs a user-provided handler written in a user-chosen high-level language.

\end{comment}



\subsection{Open-Source Benchmarking  for Serverless Systems and Architectural Research}

\boris{Would be good to explicitly state that (a) there is no open-source serverless infrastructure for at-scale experiments, and (b) the infrastructure used in existing work is incomplete/simplified. Not sure where to do it, but perhaps right in this section.}

The datacenter-scale architecture of serverless systems makes it imperative to carefully consider and model all the components of the distributed serverless infrastructure. Serverless research infrastructure needs to meet a number of key requirements that are representativeness in its architecture and each of the software components and the communication fabrics, robust evaluation methodology, and extensibility for fast prototyping of various research ideas. 

We present a complete end-to-end open-source infrastructure for serverless that achieves all of the aforementioned goals by building around the de facto standard plugin-based containerd framework~\cite{containerd:industry} for host orchestration, leveraging available industrial standard components and fabrics (including the Firecracker hypervisor~\cite{agache:firecracker} and gRPC communication framework~\cite{google:grpc}) while re-using and packaging functions from the state-of-the-art serverless function benchmark suite~\cite{kim:functionbench,kim:practical}. 

The infrastructure comprises loosely coupled modules for each of the essential components of the serverless architecture, seeking to enable innovation in any of these components with careful evaluation of the chosen components' implications on the end-to-end serverless system performance. All standard components are available as public forks of the industry and open-source community maintained repositories to allow seemless upgrades to the state-of-the-art continuously released features.

\marios{Think of adding a second figure with the components we used; reinforce the coordinator contribution}
The \textbf{centralized experiment coordinator service} implements load and latency measurement methodology. We build this custom component to drive all other infrastructure components through experiment phases, such as initial configuration and deployment of the distributed components, overall system warm-up phase, and stepping through a number of measurement phases (e.g., sweeping the load traffic, memory pressure, etc.). The components are coordinated via low latency gRPC fabric that allows fine-grain sub-millisecond coordination.
The coordinator also plays the role of the simplified worker manager, setting up long-living connections between the front-end and the workers. In future, we plan to delegate the worker manager's role to Kubernetes~\cite{k8s}, which is a de facto industry-standard cluster orchestrator.

\textbf{Front-end} is represented by a configurable number of custom load and latency clients that drive the invocation traffic and measure the end-to-end response latency of the deployed functions. 
Each load client drives its fraction of the load in an open loop, issuing invocation requests to functions according to functions popularity distribution (e.g., to model hot and cold functions as in a realistic deployment~\cite{shahrad:serverless}) and the target load. The latency clients issue one invocation request at a time, waiting for its completion, to exclude client-side queueing effects. Clients periodically report their throughput and latency measurements to the coordinator that aggregates the measured results.

The \textbf{ worker orchestration framework} includes containerd for managing function instances and the custom-build gateway service that mediates both the control and data plane inbound and outbound requests. 
We choose containerd because of its modularity, as nearly all containerd components are independent plugins, and wide support of the open-source and industrial communities led by Cloud Native Computing Foundation ~\cite{cncf,kata:containers,fc-ctrd:deep-dive,ctrd:gvisor}. This infrastructure supports different types of sandboxes, including virtual machines~\cite{agache:firecracker,kata:containers} and containers~\cite{opencontainers}, and common container toolchains. The supported toolchains provide a wide range of container primitives for deployment (e.g., container image layers), function instances isolation (e.g., network and filesystem namespaces along with system call whitelisting), host resources management (including network, CPU and memory limits per container), as well as logging and monitoring~\cite{prometheus}. 
We adopt the public containerd fork~\cite{fc-ctrd:github}, that is maintained by Amazon Firecracker engineers, that includes firecracker-specific shim components, both external and internal to the instance's sandbox. We showcase the flexibility of containerd by extending the original fork with the latest Firecracker feature that is virtual machine snapshots~\cite{fc:snaps} \boris{This is confusing. You have an official Amazon fork of Firecracker and you say you extend the fork with a Firecracker feature -- but why is that feature not in your fork?}.
%Amazon Firecracker~\cite{agache:firecracker}, Google gVisor~\cite{google:gvisor}), cluster orchestrators (e.g., Kubernetes~\cite{k8s}), and standard Open Container Initiative images~\cite{opencontainers}. 

For \textbf{sandbox} we choose Amazon Firecracker~\cite{agache:firecracker} that powers up Amazon Lambda and Fargate services but is widely adopted by other cloud providers, including Baidu AI Cloud~\cite{baidu:kata}, OpenNebula~\cite{opennebula:firework}, and WeaveWorks~\cite{weave:firekube}. A Firecracker sandbox is a full-blown virtual machine that runs a minimalist Linux kernel that delivers high security and isolation while providing performance close to container-based solutions.

\textbf{Gateway service} is implemented as a custom scalable multi-threaded gRPC-based software service that mediates both the control plane and data plane requests. We design the gateway service as a seamless extension of containerd that communicates to other components -- namely the coordinator, clients, containerd, and the function instances -- using the gRPC fabric that is the default choice for the existing containerd components.

\input{floats/tbl_functionbench}

\textbf{Functions} are implemented as gRPC-based single-threaded servers that run inside their corresponding sandboxes \boris{Need to explain/justify the single-thread aspect. Reviewers that are not knowledgable might think that vHive is not sufficiently 'serious' because it doesn't support multi-threading.}. The current release of vHive includes a simple \texttt{helloworld} function and eight functions from FunctionBench~\cite{kim:functionbench,kim:practical}, a representative suite of serverless functions written in Python that includes web processing, cryptography, image processing, machine learning models serving and training (Table~\ref{tbl:functionbench}). 
%a minimal helloworld function, web rendering, text encryption, image transformation, JSON serialization and de-serialization, three ML serving functions of different classes and frameworks, and client review predictor training (Table~\ref{tbl:functionbench}). 
FunctionBench originally distributes its benchmarks as collections of Python scripts; we wrapped these into gRPC servers deployed on top of Linux Alpine and containerized them into Docker/OCI images. \boris{I rewrote the last sentence - please check.}
%where each image comprises the function code packaged on top of Linux Alpine distribution. 


%>>>>>>>>>>>>>>>>>>>
\begin{comment}

\subsubsection{Requirements for a systems research platform}
\begin{itemize}
    \item Representativeness: Architecture and operation that are similar to those of industrial leaders, including both control and data planes, production-grade components and protocols, host and guest resources management, and virtualization (\S\ref{sec:serverless101}).
    \item End-to-end distributed system evaluation: robust methodology with high load and latency clients that drive the load towards both the control and data plane.
    \item Flexible and fast prototyping: plugin-based architecture based on industry-standard and industry-leading software components (containerd, gRPC), extensive test coverage.
\end{itemize}

\textbf{Load and latency clients as Front-end.} Open-loop load clients and close-loop latency clients based on gRPC~\cite{google:grpc}. Data path connects to the Gateway service. 

\textbf{Cluster scheduling.} TBD: our infra is compliant but right now it does not have cluster scheduling components. Long-term goal is to integrate our custom gateway service (see below) with containerd-cri plugin that would make it compatible with Kubernetes.

\textbf{Gateway service.} Custom Golang-based high-performance service that acts as a gRPC-level software router and a function instances manager via commands to the host orchestrator. Acts as a bridge between the universe of functions and and function instances. 
%Can be both stand-alone and co-located with each worker.

\textbf{Containerd as host orchestrator.} OCI and CRI/Kubernetes compliant, support for various sandboxes (runtimes), metrics collection with Prometheus. Support for overlay-based disk snapshots, virtual network configuration (incl., CNI), per-VM external and internal shim processes, connected with gRPC (ttrpc between the shims).

\textbf{Sandbox.} We chose Firecracker hypervisor as one of the leading solutions, used by AWS, Alibaba Cloud, Baidu AI Cloud~\cite{baidu:kata}, OpenNebula~\cite{opennebula:firework}, WeaveWorks~\cite{weave:firekube}. The sandbox runs a minimal Linux kernel

\textbf{Function server.} Deployed as an OCI-compliant container image that containerd supplies to the guest OS as a virtual disk to be mounted during guest OS boot process. The image comprises a gRPC server that wraps a user-provided function in a user-chosen language to serve RPCs that come from the clients (i.e., the Front-end fleet) via the Gateway service.

\textbf{Workloads aka Functions.} We adopt eight functions, from FunctionBench~\cite{kim:functionbench,kim:practical}, that cover a wide range of serverless use cases: image rotation, web rendering, encryption, json serialization, various ML serving and training. We integrate all workloads with a Python gRPC server. Functions are deployed in Alpine Linux images, commonly used in Serverless and Edge deployments due to its security and image-size advantages~\cite{alpine:containers}.

\end{comment}
%<<<<<<<<<<<<<<<<<<<<<<<<<<<<<





==> old versions/4-design.tex <==
\section{\tac{}: \tnameabs{} Orchestrator}
\label{sec:design}

Acknowledging the potential \boris{potential for what? This is vague} arising from the above memory analysis, we design \tname{} (\tac), a system to accelerate the boot time of functions from a snapshot. \tac{} records the hot pages used by a function during its execution and eagerly prefetches these pages into memory right before  function invocation.

When designing \tac{} we set the following design goals:
i) User codebase should remain agnostic to \tac{};
ii) \tac{} should be independent of the underlying FaaS technology;
iii) \tac{} should be entirely implemented in userspace to avoid kernel modifications; \boris{these are really good. Should highlight these as design principles/contributions in the Intro.}

\subsection{Overview}
\label{sec:design_overview}
% reap steps
%\boris{I don't like saying that snapshot creation is part of REAP. It's the baseline functionality, hence is a given and REAP simply builds on that.}
\dmitrii{{\tac} builds upon the original snapshot functionality, provided by Firecracker, and assumes the snapshot files are available, by introducing functionality for two phases: record and prefetch. The first, record, phase happens once upon the first invocation, recording the working set of pages that a function instances accesses during an invocation. The prefetch phase happen once for each function invocation after the record phase.
}
%\tac{}'s functionality is split into three distinct phases: the snapshot creation phase, the record phase, and the prefetch phase.

%The first two phases happen once for each function, while the prefetch phase happens once every function invocation. Since \tac{} builds and improves upon snapshots, the first step is to take a snapshot of the runtime right before executing the function. As with vanilla snapshoting booting directly the snapshot rather than initializing the environment every time improves function start up times.

%The next phase, 
The record phase, happens during the first invocation of a function and its goal is to identify the memory pages the function requires for its execution.
The key insight here is that, as seen in Figure~\ref{fig:char_pages_reuse}, those pages are highly likely to be reused in future function invocations, while the overall memory size of these pages is expected to be significantly smaller than the snapshot size and the memory footprint of the function invocation since boot time.

After identifying those pages, \tac{} prefetches them to memory from disk right before the function invocation every time this specific function has to be executed in the future during the prefetch phase.
This way despite the function not occupying space in memory, it does not pay the cold-boot performance price since pages that are highly likely to be access are going to be warm. \boris{Unless you can show that REAP reduces the exec latency to that of a warm function, this is overclaiming. You are reducing cold boot latency, but not eliminating it.}

\subsection{Implementation}
\label{sec:implementation}

\boris{I'm not a fan of this section. First of all, this is not Challenges - these are simply design decisions. Secondly, there's an abstraction gap -- the prev subsection is too high level, and this one is too low level. You need to beef up the previous section by adding a walk-through of the system (aided by a figure) that explains REAP. It should show that \\
(a) a snapshot has only a small number of pages resident in memory during exec; \\
(b) these pages are compacted into a trace and recorded on disk; \\
(c) the traces is read from start to finish at once into mem; \\
(d) the page table is eagerly populated. 

Keep the discussion high-level without getting into mechanisms (user pagefaults, ioctl, etc). But make sure that you highlight the key principles: \\
- small working set implies compact trace \\
- reading trace at once achieves high disk BW \\
- installing pages in bulk amortizes the page fault overhead.

Lastly, we need to make sure that disk BW and the cost of ioctls are clearly identified as problems in Sec 2.

After the above is done, you can dive directly into implementation. There you, need to say explain up-front that the key to your design is taking advantage of user-level pagefaults, which enable bulk install etc without kernel modifications.}

The above described an abstract view of \tac{}.
We, now, identify the two main challenges behind \tac{} and explain how we dealt with them respecting our initial design goals.
The first challenge is how to capture the function working set, namely the majority of the memory pages used during execution while remaining agnostic to the user code and outside the kernel space.
The second challenge, and the one which will define the benefit of our proposal, is how to restore the working set from disk in a timely and fast manner.

\paragraph{Record phase:}
\tac{} needs to capture all pages accessed during the function invocation after the snapshot boot during the record phase and do so in a kernel-agnostic and source-code-agnostic manner.
\tac{} leverages a userspace pagefault handler for that.
%Every snapshot is stored in a file that corresponds to the entire guest memory.
\dmitrii{A VM snapshot contains a file that stores the contents of the entire guest memory.}
\dmitrii{To load a VM from a snapshot, the hypervisor maps this guest-memory file as an anonymous virtual memory region, restores the VMM and emulation layer state, and resumes the VM to start processing a function invocation. Every access to the guest memory raises a page fault that needs to be handled and recorded in userspace.
}
%Accessing a page from the snapshot for the first causes a pagefault that is logged and handled in userspace.

%Every function is associated with a \emph{monitor} process that is in charge of handling user pagefaults.
\dmitrii{The gateway service allocates a \emph{monitor} thread (implemented as a light-weight goroutine) per function instance that is responsible for handling user page faults that are triggered by that instance. The monitor thread maps the guest memory file, waiting for the host kernel to forward the page fault events, triggered by the instance, to the monitor. 
The monitor records the offset in the guest memory file that corresponds to the faulting virtual address, then installing the page into the guest memory region of the instance by issuing an \texttt{ioctl} system call to the host kernel.
This file offsets recording procedure increases the function invocation time as compared to the baseline snapshots \boris{can you say by how much (e.g., 10\%?) and add a forward pointer to Eval}, due to the page faults forwarding through the host kernel, but only penalizes the first function invocation. Together the recorded offsets correspond to the working set of pages, inside the guest-memory file, that a function instance needs to process an invocation.
\boris{This sounds like only offsets are recorded. In reality, the actual memory pages are stored in the trace. Clarify. Also, need to say that the file is flushed to disk once the function completes.}
}
%The \emph{monitor} also maps the guest memory file and is notified through a \texttt{userfaultfd}~\cite{man:userfaultfd} every time the function execution causes a page fault.
%The monitor records the address of the page the function tried to access and installs the mapping through an \texttt{ioctl}.
%The above process increases the function execution time but only penalises the first function invocation.


\paragraph{Prefetch phase:}
\dmitrii{NOTE, need to say that: load VMM is overlapped with fetch so this latency is off the critical path}
\dmitrii{The {\tac} monitor uses the recorded offsets to prefetch the working set memory pages from the guest memory file, located on disk, into its own memory at the time of the function invocation, serving the subsequent page faults that happen during a function invocation. While most of the page faults correspond to the recorded offsets, a small fraction of the page faults would require bringing extra pages from the guest memory file before serving.
}

%\tac{} uses the \texttt{monitor} process also after the first function invocation.
%The \texttt{monitor} is in charge of prefetching the working set memory pages from the guest memory file located on disk into its own memory at the time of the function invocation and serve the subsequent pagefaults happening during the function execution. 
%If the faulted page belongs to the working set installs the new mapping directly else first reads the guest memory file and install the mapping.

\tac{}'s efficiency depends entirely on the performance of the prefetch phase.
For that we design a few optimisation steps that go after minimizing the disk access time by leveraging the full SSD bandwidth and reducing the cost of \dmitrii{installing the pages into the guest memory that requires issuing} \texttt{ioctl} system calls.

We consider four different \tac{} configurations that gradually apply the optimization steps.
The baseline \tac{} eagerly reads the randomly scattered pages from the guest memory file into a buffer in the monitor's memory and lazily installs each page when the page fault to its corresponding address happens during the function invocation, thus avoiding disk accesses during the function invocation.
We call this configuration \texttt{eager-read-lazy-install (ERLI)}.
The first optimization step is to eagerly install the pages in the working set by performing all the \texttt{ioctl} calls at once at the function invocation time.
We call this configuration \texttt{eager-read-eager-install (EREI)}.
\texttt{EREI} performs one \texttt{ioctl} per page in the working set.

%\dmitrii{Figure~\ref{fig:char_pages_reuse}, though, identifies that there is an opportunity to coalesce distinct pages into a number of contiguous memory regions.} This way \tac{} can reduce \dmitrii{the number of \texttt{ioctl} calls that are necessary for the eager installation, performing a single} call per contiguous memory region.
%\dmitrii{In this configuration, the monitor coalesces both the read system calls to fetch the guest memory file into a memory buffer and the \texttt{ioctl} calls to install the regions.} We call this version \texttt{coalesce-eager-read-eager-install (CEREI)}.

Finally, all the above configurations require random disk accesses while reading the working set pages, thus not taking advantage of the full disk bandwidth, while requiring several read system calls to achieve so.
To achieve so, \tac{} condenses the working set pages into a small file right after the record phase.
This way \tac{} can read the entire working set file with a single read system call. 
\dmitrii{To leverage the whole available SSD bandwidth, we use \texttt{O\_DIRECT} flag when reading the working set file into a memory buffer to bypass the host OS' page cache, allowing to increase the SSD by 2.6$\times$.}
We call this version \texttt{condense-coalesce-eager-read-eager-install (CCEREI)}.


%\dmitrii{it should be more like an SSD throughput argument rather than latency. may want to say instead: the goal is to saturate available SSD BW. since PFs come one-by-one serially, one cannot benefit from SSD's internal parallelism. Example, peak throughput of our SATA3 SSD is 900MB/s but with 1 outstanding IO, it drops to 30MB/s}
 
 
 
 
 
 
 
 
 
 
\begin{comment}

\subsection{Implementation}
\label{sec:implementation}

\dmitrii{Design: 3 phases: boot \& snap creation, record, prefetch. Centralized design inside the the trusted orchestrator code.

Implementation: proactive prefetch of the recorded pages, parallelism for high multi-tenancy, amortise disk accesses by using a condensed WS file. Discussion around disaggregated storage of WS and/or guest memory file vs. local storage. Probably, having th WS file locally, guest mem remotely makes most sense.
}


Design principles

\begin{itemize}
    \item ...
    \item Security: SSD bandwidth is a limited shared resource, hence access to it needs to be mediated by the trusted software (the orchestrator).
\end{itemize}

\boris{Discussion: our design description assumes local snapshot storage. REAP can also work with disaggregated storage. Very briefly explain.}
\dmitrii{discuss a hybrid solution with a working set locally and the full memory file remotely}
\end{comment}


==> old versions/char_e2e.tex <==
\begin{figure}[t]
\centering
\subfloat[Boot \textbf{ETA: 7.08}]{
    \includegraphics[width=0.98\columnwidth]{figs/blank.png}
    \label{fig:e2e_boot}}
\newline
\centering

\subfloat[Snap \textbf{ETA: 7.08}]{
    \includegraphics[width=0.98\columnwidth]{figs/blank.png}
    \label{fig:e2e_snap}}
\caption{Latency/throughput of serverless server (X\% cold-start ratio).}
\label{fig:char_e2e}
\end{figure}

==> old versions/design_idea.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/reap_idea.pdf}
\caption{Working set installation with {\tac}.}
\label{fig:reap_idea}
\end{figure}
